HiPO: Hybrid Policy Optimization for Dynamic Reasoning in LLMs

Large Language Models (LLMs) increasingly rely on Chain-of-Thought (CoT) reasoning to improve accuracy on complex tasks. However, always generating lengthy reasoning traces is inefficient, leading to excessive token usage and higher inference costs. This paper introduces the Hybrid Policy Optimization (i.e., HiPO), a framework for adaptive reasoning control that enables LLMs to selectively decide when to engage in detailed reasoning (Think-on) and when to respond directly (Think-off). Specifically, HiPO combines a hybrid data pipelineproviding paired Think-on and Think-off responseswith a hybrid reinforcement learning reward system that balances accuracy and efficiency while avoiding over-reliance on detailed reasoning. Experiments across mathematics and coding benchmarks demonstrate that HiPO can substantially reduce token length while maintaining or improving accuracy. Finally, we hope HiPO a can be a principled approach for efficient adaptive reasoning, advancing the deployment of reasoning-oriented LLMs in real-world, resource-sensitive settings.

==> Tables/more_models.tex <==
\begin{table}[H]
\centering
\resizebox{\linewidth}{!}{
    \setlength{\tabcolsep}{8pt}
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
                                                             & \multicolumn{2}{c|}{AutoThink_{Think-on}}             & \multicolumn{2}{c|}{AutoThink}             & \multicolumn{2}{c|}{GRPO_{Think-on}} & \multicolumn{2}{c|}{GRPO_{AutoThink}}    & \multicolumn{2}{c|}{Our-RL_{AutoThink}}           \\
\multirow{-2}{*}{Method}                                     & Acc                & Length             & Acc                & Length             & Acc                   & Length             & Acc                   & Length             & Acc                & Length       \\ \midrule
\multicolumn{15}{l}{\textit{Qwen3-8B}}                                                                                                      \\ \midrule
AIME2024                               & -                  & -                  & -                  & -                  & -                     & -                  & -                     & -                  & -                  & -                      \\
AIME2025                                                   & -                  & -                  & -                  & -                  & -                     & -                  & -                     & -                  & -       & -                 \\
ICB                                                          & -                  & -                  & -                  & -                  & -                     & -                  & -                     & -                  & -         & -              \\
Humaneval                                                          & -                  & -                  & -                  & -                  & -                     & -                  & -                     & -                  & -       & -      \\
GSM8K                                                          & -                  & -                  & -                  & -                  & -                     & -                  & -                     & -                  & -           & -        \\
Prm800K                                                          & -                  & -                  & -                  & -                  & -                     & -                  & -                     & -                  & -            & -         \\
Average                                                    & -                  & -                  & -                  & -                  & -                     & -                  & -                     & -                  & -              & -           \\
\end{tabular} 
}
\caption{Accuracy (Acc) and response length (Length) of different methods on six benchmarks. The best and second results are bolded and underlined, respectively.}
\label{tab:main}
\end{table}
